Cosmogenic activation of sodium iodide

The production of radioactive isotopes by interactions of cosmic-ray particles with sodium iodide (NaI) crystals can produce radioactive backgrounds in detectors used to search for rare events. Through controlled irradiation of NaI crystals with a neutron beam that matches the cosmic-ray neutron spectrum, followed by direct counting and fitting the resulting spectrum across a broad range of energies, we determined the integrated production rate of several long-lived radioisotopes. The measurements were then extrapolated to determine the sea-level cosmogenic neutron activation rate, including the first experimental determination of the tritium production rate: $(80 \pm 21)$ atoms/kg/day. These results will help constrain background estimates and determine the maximum time that NaI-based detectors can remain unshielded above ground before cosmogenic backgrounds impact the sensitivity of next-generation experiments.

==> outline.tex <==
\newpage
\setcounter{section}{0}
\section  {Introduction - Liang, Greg, Will}
\begin{itemize}
    \item Cosmic rays as backgrounds for rare-events searches
    \item DM searches with NaI (motivation, different experiments)
    \item Dominant backgrounds
    \item Lack of measurements
    \item Outline of paper
\end{itemize}
\section {Cosmogenic Radioisotopes - Richard, Yi Yi, Lindsey}
\begin{itemize}
    \item Discussion of possible cosmogenic isotopes
    \item List of isotopes relevant for DM experiments
\end{itemize}
\subsection {\trit~Production}
\begin{itemize}
    \item Half-life, decay, energy
    \item Nuclear production
    \item Existing cross-section measurements
\end{itemize}
\subsection {\cad~Production}
\begin{itemize}
    \item Half-life, decay, energy  
    \item Nuclear production
    \item Existing cross-section measurements
\end{itemize}
\section {Other isotope~Production (individually)}
\begin{itemize}
    \item Half-life, decay, energy  
    \item Nuclear production
    \item Existing cross-section measurements
\end{itemize}
\section {Beam Exposure}
\subsection {NaI crystals - Richard, Lindsey}
\begin{itemize}
    \item Description, Size, thickness, purity
    \item Radiation damage concerns
\end{itemize}
\subsection {LANSCE Beam - Steve}
\begin{itemize}
    \item Facility, Beam, Energy, Target \cite{lisowski2006alamos}
    \item Fission Chamber, Fission Cross-Section uncertainty
    \item Energy (TOF)
\end{itemize}
\subsection {Exposure - Liang, Richard}
\begin{itemize}
    \item Dates, Collimation
    \item Radiation damage checks
    \item Total Fluence and uncertainty
    \item Cooldown and shipping
\end{itemize}
\subsection {Target Fluence - Raymond} 
\begin{itemize}
    \item Geant4 geometry and beam simulation
    \item Fluence through each target
    \item Beam alignment uncertainty
\end{itemize}
\section {Counting}
\subsection {Ge Counting? - Greg/Yi Yi}
\begin{itemize}
    \item LANL Ge counter setup
    \item Calibrations?
    \item Energy spectra
    \item Results
    \item Half-life corrections
    \item Uncertainty estimations
\end{itemize}
\subsection {NaI Counting - Will}
\begin{itemize}
    \item Brief description of setup and DAQ
    \item Event Reconstruction
    \item Background Runs
    \item External Source Calibrations
    \item Energy Spectra (for different crystals)
    \item Light yield and resolution (compare with unirradiated?)
    \item Time Evolution
\end{itemize}
\subsection {Simulations and Fitting - Yi Yi, Lindsey}
\begin{itemize}
    \item G4 setup (event distribution, isotopes)
    \item Applying non-linearity to individual deposits
    \item Handling of decay daughters
    \item Matching sim with data (for non-fit parameters)
    \item Fitting (software, minimization, likelihood)
    \item Results (goodness of fit, time evolution)
    \item Half-life corrections
    \item Uncertainty estimations
\end{itemize}

\section {Production Rate}
\begin{itemize}
    \item Cross-Section Model Predictions - Richard 
    \item Ejection and Implantation - Raymond 
    \item Comparison to Measurements - Richard 
\end{itemize}

\section{Cosmogenic Activation - Richard}
\begin{itemize}
    \item Cosmic neutron spectrum
    \item Scaling experimental results
    \item Final sea-level fast neutron production rates 
\end{itemize}

\section{Alternate Production Mechanisms}
\begin{itemize}
    \item Production from protons
    \item Any other mechanisms?
\end{itemize}

\section {Discussion}

